Challenges and strategies for running controlled crowdsourcing experiments

This paper reports on the challenges and lessons we learned while running controlled experiments in crowdsourcing platforms. Crowdsourcing is becoming an attractive technique to engage a diverse and large pool of subjects in experimental research, allowing researchers to achieve levels of scale and completion times that would otherwise not be feasible in lab settings. However, the scale and flexibility comes at the cost of multiple and sometimes unknown sources of bias and confounding factors that arise from technical limitations of crowdsourcing platforms and from the challenges of running controlled experiments in the "wild". In this paper, we take our experience in running systematic evaluations of task design as a motivating example to explore, describe, and quantify the potential impact of running uncontrolled crowdsourcing experiments and derive possible coping strategies. Among the challenges identified, we can mention sampling bias, controlling the assignment of subjects to experimental conditions, learning effects, and reliability of crowdsourcing results. According to our empirical studies, the impact of potential biases and confounding factors can amount to a 38\% loss in the utility of the data collected in uncontrolled settings; and it can significantly change the outcome of experiments. These issues ultimately inspired us to implement CrowdHub, a system that sits on top of major crowdsourcing platforms and allows researchers and practitioners to run controlled crowdsourcing projects.

==> sections/tmp-background.tex <==
% notes for Background

% structure 
% 0. gist
% 1. task design as a multi-dimensional challenge. show the many things that need to be configured and how these impact performance, ending the paragraph by saying that these tend to be a laborious trial-and-error process.
% 2. running studies on crowdsourcing platforms and how hard it is.
% 3. bias in crowdsourcing derived from task design and "uncontrolled aspects of it".
% 4. a paragraph summarizing related tooling that I describe in the related work.


%%% -------------------------------------- %%% %%% -------------------------------------- %%% 

% Background

% 1. task design as a multi-dimensional challenge. show the many things that need to be configured and how these impact performance, ending the paragraph by saying that these tend to be a laborious trial-and-error process.
[Task design attributes and their impact on the actual outcome.]



% task interface: instructions and their impact on performance
%%%
Confusing the Crowd: Task Instruction Quality on Amazon Mechanical Turk \cite{DBLP:conf/hcomp/WuQ17}

Task instruction quality is widely presumed to affect outcomes, such as accuracy, throughput, trust, and worker satisfaction.

Without a clear specification of what information is requested, and how to produce it, workers can hardly be expected to produce consistently good quality results

This paper presents a multidimensional analysis of task instruction quality.

Besides communicating a request, task interfaces also form a semi-formal contract between the worker and requester.

they contributed Actual effects of specific best practices on desired out- comes (e.g., accuracy, worker acceptability, etc.).

Results of the experiments show that (a) adherence to best practices can affect outcome, but that (b) workers are more resilient to flaws in task quality than current popular belief might suggest.

Unclear instructions are often cited as a main challenge for crowd workers.

that task clarity impacts workers’ acceptance of a task (Schulze et al. 2011). \cite{DBLP:conf/ecis/SchulzeSGKS11}

Poorly designed instructions affect the result quality \cite{DBLP:conf/cscw/KitturNBGSZLH13}

The design here has a broader meaning, which not only refers to the interface design but also includes the task mechanics such as when to post the task and how to filter the workers.

One insight was that worker uptake—the proportion of workers who accept the task, relative to those who viewed it—is higher for short tasks. -- so there is also a tradeoff in making a task very clear but keeping it short since it affects latency. 


%%%
Clarity is a Worthwhile Quality: On the Role of Task Clarity in Microtask Crowdsourcing \cite{DBLP:conf/ht/GadirajuYB17}

In this paper we highlight the role of clarity as a characterising property of tasks in crowdsourcing.

We show that task clarity is coherently perceived by crowd workers, and is affected by the type of the task

Poor formulation of tasks has clear consequences: to compensate for a lack of alternatives in the marketplace, workers often attempt the execution of tasks despite a sub-optimal understanding of the work to be done.

The survey involved 100 workers, and clearly highlights that workers confront unclear tasks on a regular basis.

Poor task formulation thereby greatly hinders the progress of workers’ in obtaining rewards, and in building up a good reputation.

With an extensive study we revealed that clarity is coherently perceived by workers, and that it varies by the task type

In conclusion, we demonstrated the importance of clarity as an explicit property of microwork crowdsourcing tasks.


%%%
Effective Crowd Annotation for Relation Extraction \cite{DBLP:conf/naacl/LiuSBLLW16}

they propose an training protocol.
Gated Instruction, which combines an interactive tutorial, feedback to correct errors during training, and improved screening

By carefully de- signing a quality-controlled crowdsourcing work- flow that uses Gated Instruction (GI), we are able to create much more accurate annotations than those produced by previous crowdsourcing methods

The effectiveness of crowdsourcing is dependent on a number of human factor



%%%
WingIt: Efficient Refinement of Unclear Task Instructions \cite{DBLP:conf/hcomp/ManamQ18}


Crowdsourcing has the inherent potential to shift tedious work from requesters with limited time (or patience) to an on-demand workforce.

However, the time saved by requesters is offset by the time they must spend preparing instructions and refining them to address the ambiguities that typically arise.

This paper presents a set of methods that enable workers to cope with unclear or ambiguous instructions and produce high quality results with minimal reliance on the requester

Designing clear instructions that reliably elicit accurate results requires time and attention. Several iterations may be required, especially for tasks with intricate requirements.

there have been several instances where workers were not able to complete a task or submitted a task with incorrect results due to ambiguous or sloppy instructions.


Kittur et al. suggested improving task de- sign through better communication as one of the crucial next steps in designing the future crowdsourcing solutions \cite{DBLP:conf/cscw/KitturNBGSZLH13}.

WingIt proposes another way to improve the quality of work via interaction between worker and requester when the requester is active. In the situation of an inactive requester, we consider an iterative workflow, allowing workers to col- laborate and improve answers from previous workers

When a worker encounters an ambiguity, they can ask for clarification in the form of a question ("Q&A") or a direct revision to the instructions ("Edit"). 
[both actions can be synchronous or async]


[the interesting thing here is that workers play a role in improving the instructions, things they can suggest editions.]


Comparing WingIt to a traditional approach demonstrates that WingIt can improve the quality of results and decrease the effort of requesters in creating comprehensive instructions that leave no room for subjective assessment.

We also found that workers are more interested in asking questions or making edits to the tasks in the presence of a requester





% task interface: supporting workers to improve perf
%%
Cognitively inspired task design to improve user performance on crowdsourcing platforms \cite{DBLP:conf/chi/SampathRI14}

We investigate here how improving the presentation of the task itself by using cognitively inspired features affects the performance of crowd workers


We claim that the use of cognitively inspired features for task design is a powerful technique for maximizing the performance of crowd workers.

We focused here on the form-digitization task to demonstrate the efficacy of cognitive principles to task design.

we demonstrated that different task presentations affect crowd performance significantly [improving accuracy]


%%
Crowdsourcing Annotations for Websites' Privacy Policies: Can It Really Work? \cite{Wilson2016WWW}


little attention has been devoted to studying the ac- curacy and scalability of crowdsourced privacy policy annotations

Our results suggest that, if carefully deployed, crowdsourcing can indeed result in the generation of non-trivial annotations and can also help identify elements of ambiguity in policies. 

We further introduce and evaluate a method to improve the annotation process by predicting and highlighting paragraphs relevant to specific data practices.


we investigate the feasibility of crowdsourcing privacy policy annotations and explore how the efficiency of crowd workers can be enhanced by predicting and highlighting policy paragraphs that are relevant to specific data practices

[they show that highlighting could improve productivity (e.g., effort) but it does not affect the accuracy]



%%
our paper \cite{ramirez2019}








% besides task interface, we have
%
reward configuration 
%%%    
Fair Work: Crowd Work Minimum Wage with One Line of Code \cite{Whiting2019FairWC} 


Accurate task pricing in microtask marketplaces requires sub- stantial effort via trial and error, contributing to a pattern of worker underpayment

In response, we introduce Fair Work, enabling requesters to automatically pay their workers mini- mum wage by adding a one-line script tag to their task HTML on Amazon Mechanical Turk.



%%%
Incentivizing High Quality Crowdwork \cite{DBLP:conf/www/HoSSV15} 

We study the causal effects of financial incentives on the quality of crowdwork


We focus on performance-based payments (PBPs), bonus payments awarded to workers for pro- ducing high quality work.

[they run experiments on AMT]

We provide examples of tasks for which PBPs do improve quality. 

We also present examples of tasks for which PBPs do not improve quality

Our results suggest that for PBPs to improve quality, the task must be effort-responsive: the task must allow workers to produce higher quality work by exerting more e↵ort.


Crowdsourcing markets are used to conduct user studies [22], run behavioral experiments [18, 28], collect data [17, 35], test or even build business applications [1, 31], and more.


In this paper, we study the use of financial incentives to encourage high quality crowdwork on Amazon Mechanical Turk.

We design and run experiments with the goal of understanding not just whether PBPs improve work quality for a specific task or bonus size, but when, why, and where they improve work quality.

We identify properties of the payment, payment structure, and the task itself that make PBPs effective.


We have shown that PBPs incentivize higher quality crowd- work on two specific tasks, proofreading and spotting differences in images.


We find that PBPs can improve the quality of submit- ted work for some tasks, but are not likely to for others. We identify the extent to which a task is effort-responsive as a potential important reason for whether or not PBPs work for this task.


%%%
When Does More Money Work? Examining the Role of Perceived Fairness in Pay on the Performance Quality of Crowdworkers\cite{DBLP:conf/icwsm/YeYR17}


perceived fairness in pay (PFP)

We examine whether PFP mediates the impact of payment amount on the performance quality of crowdworkers

We conducted a field experiment with 152 crowdworkers performing a button- clicking (BC) task and an instructional manipulation check (IMC) task

PFP mediated the impact of payment amount on performance quality in the BC task but not in the IMC task.

Results suggest that PFP can help us better understand the relationship between payment and per- formance quality in crowdsourcing

We propose that in crowdsourcing, when crowdworkers believe they are being paid fairly they per- form better.

[they used AMT]


Via the lens of perceived fairness in pay, this paper sought to extend our understanding of the relationship be- tween financial incentives and crowdworkers’ performance.



in order to rule out potential cultural differences (Shaw, Horton, and Chen 2011).
    Shaw, Horton, and Chen 2011: Designing Incentives for Inexpert Human Raters


this study broadens the discussion on pay and crowd work to include satisfaction and task time

When crowdworkers thought they were paid fairly, not only did they work faster, but they also were more satisfied.

[not very clear what they concluded. It seems that indeed perception of fair payment plays a role, but it is not clear to what extend.]


%%%
Designing incentives for inexpert human raters \cite{DBLP:conf/cscw/ShawHC11}

measured the effectiveness of a collection of social and financial incentive schemes for motivat- ing workers to conduct a qualitative, content analysis task.

Overall, workers performed better than chance, but results varied considerably depending on task difficulty.

We find that treatment conditions which asked workers to prospectively think about the responses of their peers — when combined with financial incentives — produced more accurate performance.


Other treatments generally had weak effects on quality

[this is the "negative" effect of monetary incentives that was mentioned in \cite{DBLP:conf/www/HoSSV15} ]


Workers in India performed significantly worse than US workers, regardless of treatment group.
[this also highlights the importance of controlling demographics].


[ran on AMT]


%%%
Financial incentives and the performance of crowds \cite{DBLP:journals/sigkdd/MasonW09}

Here we investigate the effect of compensation on performance in the context of two experiments, conducted on Amazon’s Mechanical Turk (AMT)


we note that previous studies have also found positive effects of financial incentives on quantity of work performed but no effect on quality


Our main findings are twofold: first, we found that increased payments increased the quantity of work performed, but not its quality; and second, that the particular design of the compensation scheme (a quota scheme versus a piece rate, for example) can have a significant effect on quality even to the point where better work can be accomplished for less pay.





%
time on tasks
%%
Crowdsourcing relevance assessments: The unexpected benefits of limiting the time to judge \cite{maddalena2016crowdsourcing} 
    
we study how the time available to express a relevance judgment affects its quality.

[CrowdFlower]

Experimental results show that it is possible to reduce the cost of crowdsourced evaluation col- lection creation by reducing the time available to perform the judgments with no loss in quality
    
    
%%
Embracing error to enable rapid crowdsourcing \cite{krishna2016embracing}

To scale and widen the applicability of crowdsourcing, we present a technique that produces ex- tremely rapid judgments for binary and categorical labels.

[they propose a mechansim for speeding up the decision process in binary/multi-class classification tasks --- for images]


We have suggested that crowdsourcing can speed up labeling by encouraging a small amount of error rather than forcing workers to avoid it.



%
optimization algorithms to derive higher-quality results

Here the idea is to show works that focus on algorithms to derive quality outcomes, which is also an equally important dimension in task design.

%%%
Quality management on amazon mechanical turk \cite{IpeirotisHCOMP2010}

Massive redundancy is expensive, increasing sig- nificantly the cost of crowdsourced solutions

we need techniques that will accurately estimate the quality of the workers, allowing for the rejection and blocking of the low-performing workers and spammers.


existing techniques cannot separate the true (un- recoverable) error rate from the (recoverable) biases that some workers exhibit.

We present algorithms that improve the existing state-of-the-art techniques, enabling the separation of bias and error.


So, naturally a question arises: How can we separate lowquality workers from high-quality, but biased, workers?



%%%
AUTOMAN: A Platform for Integrating Human-Based and Digital Computation \cite{DBLP:conf/oopsla/BarowyCBM12}


%%%
Decision-theoretic Control of Crowd-sourced Workflows \cite{DBLP:conf/aaai/DaiMW10}


% TODO: add more, e.g., Evgeny's works, etc.



---
% Instructions are vital to clearly communicate the needs of stakeholders to the workers that will undertake the task.


Task design is a crucial step in crowdsourcing projects, typically consisting of trial-and-error cycles for researchers. Task design goes beyond defining the actual task interface, involving the deployment, collection, and mechanisms for assuring the contributions from non-expert annotators meet quality objectives \cite{DBLP:journals/csur/DanielKCBA18}.
%
As such, the design of a task represents a multi-dimensional challenge for researchers, where the underlying dimensions could potentially impact the outcome of the crowdsourcing process.
%
Instructions are vital to communicating the needs of requesters since poorly defined guidelines could affect the quality of the contributions \cite{DBLP:conf/hcomp/WuQ17,DBLP:conf/cscw/KitturNBGSZLH13,DBLP:conf/ht/GadirajuYB17,DBLP:conf/naacl/LiuSBLLW16}, as well as whether workers would select the task in the first place \cite{DBLP:conf/ecis/SchulzeSGKS11} which affects the latency of the process.
%
Tasks can also vary in complexity and difficulty; thus, researchers also explored how to facilitate the job of workers by improving the task interface, showing that enriched interfaces could help in speeding up the job of workers and potentially the quality of their contributions \cite{DBLP:conf/chi/SampathRI14,Wilson2016WWW,ramirez2019}.
%
Accurate task pricing is also a relevant aspect since workers are paid for their contributions \cite{Whiting2019FairWC}, where the pricing serves as an incentive mechanism for the quantity of the contributions performed by workers \cite{DBLP:journals/sigkdd/MasonW09}, and also the quality, especially for demanding tasks \cite{DBLP:conf/www/HoSSV15}.
%
The quality could also be affected by the time workers are allowed to spend on a task \cite{maddalena2016crowdsourcing}.


---


%%% -------------------------------------- %%% %%% -------------------------------------- %%% 


















%%% -------------------------------------- %%% %%% -------------------------------------- %%% 
% 2. running studies on crowdsourcing platforms and how hard it is.

%%%
Crowdsourcing User Studies With Mechanical Turk \cite{DBLP:conf/chi/KitturCS08}

the costs involved in engaging users often requires practitioners to trade off between sample size, time requirements, and monetary costs

special care is needed in formulating tasks in order to harness the capabilities of the approach

crowdsourcing helps in running user studies and releasing researchers from the tradeoff between number of participants, time requirements and monetary costs.

Micro-task markets offer the practitioner a way to quickly access a large user pool, collect data, and compensate users with micro-payments


Mechanical Turk does not have robust support for participant assignment, making even simple between-subject designs difficult to execute.

It is possible to simply use Mechanical Turk as a recruitment device and to host the user study oneself using a simple API to send and receive participant information from Amazon.

special care must be taken in the design of the task, especially for user measurements that are subjective or qualitative


Collecting input from only a small set of participants is problematic in many design situations

small samples often lead to a lack of statistical reliability, making it difficult to determine whether one approach is more effective than another



%%%
From: Confusing the Crowd: Task Instruction Quality on Amazon Mechanical Turk \cite{DBLP:conf/hcomp/WuQ17}
even novices without expertise in interface design and crowdsourcing can participate in a freely flowing market for labor transfer. [--- This is something I could say when I close this paragraph].




%%%
From: Designing incentives for inexpert human raters  \cite{DBLP:conf/cscw/ShawHC11}
Workers in India performed significantly worse than US workers, regardless of treatment group.
[this highlights the importance of controlling demographics].


%% 
The Future of Crowd Work \cite{DBLP:conf/cscw/KitturNBGSZLH13}

we outline a framework that will enable crowd work that is complex, collaborative, and sustainable


The goal of this framework is to envision a future of crowd work that can support more complex, creative, and highly valued work




%% 
Understanding Workers, Developing Effective Tasks, and Enhancing Marketplace Dynamics- A Study of a Large Crowdsourcing Marketplace \cite{DBLP:journals/pvldb/JainSPW17}

we shed light on three crucial aspects of crowdsourcing: (1) Task design  (2) Marketplace dynamics, and (3) Worker behavior.


For the future of crowdsourcing marketplaces, it is therefore both important and timely to step back and study how these marketplaces are performing, how the requesters are making and can make best use of these marketplaces, and how workers are participating in these marketplaces in order to develop more efficient marketplaces, understand the workers’ viewpoints and make their experience less tedious, and design more effective tasks from the requester standpoint.


[what constitutes an effective task]




%%
Human Computation Must Be Reproducible \cite{DBLP:conf/www/Paritosh12}

[this paper focuses on behavioral science, particularly on content analysis and coding]

In the social and behavioral sciences, when using humans as measuring instruments, reproducibility guides the design and evaluation of experiments.

a focus on reproducibility has implications for design of task and instruc- tions, as well as for the communication of the results

In order for us to have confidence in any such criteria, the results must be reproducible, i.e., not a result of chance agreement or irreproducible human idiosyncrasies, but a reflection of the underlying properties of the questions and task instructions, on which others could agree as well.


A much stronger claim than reproducibility is validity.


the reproducibility is the extent to which a measurement gives consistent results, and the validity is the extent to which the tool measures what it claims to measure


In contrast to reproducibility, validity concerns truths

Reproducibility provides assurances that particular research results can be duplicated
validity provides assurances that claims emerging from the research are borne out in fact


We might want the results of human computation to have high validity, high utility, low cost, among other desirable characteristics. However, the results must be reproducible in order for us to measure the validity or utility to a degree better than chance.


We have found reproducibility to be a useful guide for task and guideline design. 
It is humbling how often the initial understanding of the task and guidelines turns out to lack reproducibility.

[variability in human computation: incomplete instructions, imprecise guidelines, validation data is expensive and unavailable (gold data)]


In measurement theory, reliability is the more general guarantee that the data obtained are independent of the measuring event, instrument or person
    [here we have 3 kinds of reliability: stability, reproducibility, and accuracy.]




%%
Evaluating Amazon’s Mechanical Turk as a Tool for Experimental Behavioral Research \cite{Crump2013}

relative to traditional laboratory studies, many aspects of the testing environment are not under the experimenter’s control

we attempt to empirically evaluate the fidelity of the AMT system for use in cognitive behavioral experiments

While most of replications were qualitatively successful and validated the approach of collecting data anonymously online using a web-browser, others revealed disparity between laboratory results and online results.

One challenging aspect of experimental psychology research is the constant struggle for data.


the service has been validated as a tool for conducting survey research [3,4], one-shot decision-making research [5,6], collective behavior experiments [7,8], for norming stimuli, and conducting behavioral linguistics experiments [9,10].
    
    6. Running experiments on Amazon Mechanical Turk \cite{Paolacci2010RunningEO}
    4. Amazon’s Mechanical Turk: A new source of inexpensive, yet high-quality, data? \cite{Buhrmester2011AmazonsMT}
    7. Financial incentives and the Performance of Crowds \cite{DBLP:journals/sigkdd/MasonW09}
    10. Using Amazon mechanical turk for linguistic research \cite{Schnoebelen2010UsingAM}



two key challenges for online data collection
    1. there are technical challenges in programming web-based experiment protocols and then ensuring the browser systems of the participant and experimenter support the same features.
    2. experiments where memory and timing are important are likely more sensitive to incidental aspects of the testing environment that are difficult to control online

The aim of the present paper is to validate AMT as a tool for behavioral cognitive research, with a specific focus on complex multi-trial designs.

we recommend that reviewers and editors should consider accepting behavioral experiments done on AMT as a valid methodology (applying as much scrutiny as they would apply to any behavioral paradigm)


Despite these concerns, overall, we believe AMT is a revolutionary tool for conducting experiment

% [money does not necessarily affect quality, but it DOES affect traction and latency]
While our analysis suggests that lower pay doesn’t necessarily affect the quality of the data, we have found that we can recruit participant faster and have fewer dropouts by making the study financially appealing

Most importantly, we found that testing participants’ comprehension of the instructions was critical.

dropout rates can interact in complex ways with dependent measures such as accuracy (low performing individuals may be more likely to drop out). We recommend that, perhaps unlike a typical laboratory study, all Internet experiments report dropout rates as a function of condition.


In conclusion, AMT is a promising development for experimental cognitive science research.





%%
Exploring crowd consistency in a mechanical turk survey \cite{DBLP:conf/icse/SunS16}

In this paper, we aim to explore characteristics of the worker population on Amazon’s Mechanical Turk, a popular microtask crowdsourcing environment, and measure the percentage of workers who are potentially qualified to perform software- or computer science-related tasks.

Our results show that 24\% of the study participants have a computer science or IT background and most people are payment driven when choosing tasks.


Crowdsourcing platforms like MTurk provide convenient environments for conducting empirical studies

in order to get quality experimental data, workers’ consistency should not be taken for granted

Our results show that a considerable percentage of workers have college degrees and are potentially qualified for software engineering related tasks.


Study 1 and Study 2 and observe significant differences in gender and whether participants hold a CS degree.

These results have implications for people who run studies on MTurk, illustrating a need for large sample sizes and controls for participant quality while a study is running.

[so yes, it is feasible but we need to control stuff]



%%
From: Is Once Enough? On the Extent and Content of Replications in Human-Computer Interaction

Replications have been much discussed in the literature on scientific methodology [e.g., 24,45]. Usually, replications are taken to mean the confirmation of the results of one study in a second, independent study [45]. Despite the importance of original, first discoveries in science, many have argued that there is too much emphasis on such discoveries [e.g., 20], and consequently less on replications



%%
Platform-Related Factors in Repeatability and Reproducibility of Crowdsourcing Tasks \cite{Qarout2019PlatformRelatedFI}

The datasets generated by means of crowdsourcing are, however, dependent on many factors that affect their quality.

These include, among others, the population sample bias introduced by aspects like task reward, requester reputation, and other filters introduced by the task design.

we analyse platform-related factors and study how they affect dataset characteristics by running a longitudi- nal study where we compare the reliability of results collected with repeated experiments over time and across crowdsourc- ing platforms.

1) experiments replicated across different platforms result in significantly different data quality levels.

2) the quality of data from repeated experiments over time is stable within the same platform


Using quality control mechanisms to obtain reliable results is identified as one of the main challenges in crowdsourcing (Kittur, Nickerson, and Bernstein 2013; Assis Neto and Santos 2018).

reproducing the results for identical tasks over multiple platforms has not previously been explored.

represent reliability as a measure of consistency

[run on AMT and F8]

the demographic distribution of the workers on MTurk includes mainly the US and India (Difallah, Filatova, and Ipeirotis 2018) and workers are all recruited through a unique channel


[they focus on repeatability, reproducibility, and Generalizability]

our results confirm that introducing a bonus for high-quality labels has a positive effect on labelling quality.



Based on a recent study by Difallah, Filatova, and Ipeirotis (2018), the like- lihood of having the same workers participating in future tasks is very low.



The reasons why significant differences between platforms in completion time per single task for Dataset 1 were observed could be related to language and demographics distribution of crowd workers on these platforms.


The majority of workers on MTurk are based in the US (Difallah, Filatova, and Ipeirotis 2018).

This may have led them to finish the task faster than workers in F8 who constitute a more demographically diverse group and may be from other countries around the world \cite{Qarout2019PlatformRelatedFI}.

The demographic distribution of the workers on MTurk includes mainly the US and India (Difallah, Filatova, and Ipeirotis 2018) \cite{DBLP:conf/wsdm/DifallahFI18}


%%
Evaluating online labor markets for experimental research: Amazon.com's Mechanical Turk
 % just skip


%%
The viability of crowdsourcing for survey research
    % just skip

%%
Running experiments on Amazon Mechanical Turk \cite{Paolacci2010RunningEO}


%%
Amazon’s Mechanical Turk: A new source of inexpensive, yet high-quality, data? \cite{Buhrmester2011AmazonsMT}
    % just skip


%%
Financial incentives and the Performance of Crowds \cite{DBLP:journals/sigkdd/MasonW09}
    % just skip (read it already)


%%
Using Amazon mechanical turk for linguistic research \cite{Schnoebelen2010UsingAM}
    % just skip




% The point that I want to make is that we can indeed run user studies but they are not trivial.
----
% Over the years, a [adjective] of studies [cite works that assessed the feasibility of experiments and studies] assessed the feasibility of crowdsourcing for establishing as a mechanism that goes beyond a being a facilitator for building machine learning datasets [cite Snow, GatedInstructions, and a couple more maybe], serving as an online platform for running user studies and experiments and even complex work that initially does not fit in the micro-task market [some works on interdependent task].

% cleaner version of the above.
Over the years, a vast body of work assessed the feasibility of growing the scope of crowdsourcing \cite{Paolacci2010RunningEO,Buhrmester2011AmazonsMT,DBLP:journals/sigkdd/MasonW09,Schnoebelen2010UsingAM,DBLP:conf/icse/SunS16,Crump2013} [ADD ANY MISSING ONE], expanding its application beyond serving as a tool to create machine learning datasets [citations]. Paid crowd work, through crowdsourcing platforms, establishes as a mechanism for running user studies, experiments and even complex work that initially does not fit in the microtask market [citations].
%
Naturally, the set of challenges also increases along with the scope and ambition of crowdsourcing projects. 
% I guess this could be the hook for the current paragraph that starts with "However,". and then I just mention the issue of biases that could harm the outcome.



% Over the years, crowdsourcing has evolved from a mechanism to annotate datasets for machine learning models [cite Snow, GatedInstructions, and a couple more maybe] to a [platform or another word] for sophisticated user studies and experiments.
% % 
% Researchers [\cite{DBLP:conf/chi/KitturCS08}, maybe also Evaluating online labor markets] assessed the feasibility of running user studies and experiments on AMT, identifying the underlying challenges that emerge from the lack of native support to features that are needed for running user studies and experiments.
----
%%% -------------------------------------- %%% %%% -------------------------------------- %%% 


















%%% -------------------------------------- %%% %%% -------------------------------------- %%% 
% 3. bias in crowdsourcing derived from task design and "uncontrolled aspects of it".
% The point here is that potential biases that could arise due to the lack of complete control
% and their impact on experimental results.


%%%
From: Designing incentives for inexpert human raters  \cite{DBLP:conf/cscw/ShawHC11}
Workers in India performed significantly worse than US workers, regardless of treatment group.
[this highlights the importance of controlling demographics].


r
%%%
Rehumanized Crowdsourcing: A Labeling Framework Addressing Bias and Ethics in Machine Learning \cite{DBLP:conf/chi/BarbosaC19}

[They propose a labeling framework that addresses potential biases that could emerge in the labeling process. Perhaps in the discussion of features I could mention that we architected CrowdHub in a way to plugin different pieces of logic (e.g., integrating this labeling framework).]


The process of labeling data via crowdsourcing can promote dehumanization via unfair compensation, incompatible task assignments, and unintended amplification of human biases.

[demographic bias => gender, age, country]

We propose a framework that allocates microtasks considering human factors of workers such as demographics and compensation

By routing microtasks to workers based on demographics and appropriate pay, our framework mitigates biases in the contributor sample and increases the hourly pay given to contributors.




biases introduced by the process of labeling via crowds [3, 5, 6, 8, 9, 23, 24, 26, 34]
    3. Sentiment analysis in the news \cite{DBLP:conf/lrec/BalahurSKZGHPB10}
    5. How annotation styles influence content and preferences \cite{DBLP:conf/ht/ChengC13}
    6. Accountability in algorithmic decision making \cite{DBLP:journals/cacm/Diakopoulos16}
    9. Cognitive Biases in Crowdsourcing \cite{eickhoff2018cognitive}
    23. Why gender and age prediction from tweets is hard: Lessons from a crowdsourcing experiment \cite{DBLP:conf/coling/NguyenTDGTMJ14}
    24. Social data: Biases, methodological pitfalls, and ethical boundaries \cite{DBLP:conf/wsdm/OlteanuK018}
    26. Investigating user perception of gender bias in image search: the role of sexism \cite{DBLP:conf/sigir/OtterbacherCDC18}
    34. Turkers, scholars, arafat and peace: Cultural communities and algorithmic gold standard \cite{DBLP:conf/cscw/SenGGHLNRWH15}
    
    
cultural differences in the crowd can affect algorithmic accuracy when gold-standard datasets used in machine learning applications are created via such crowds [6, 34],    

such differences may be introduced by implicit associations from different demographics

Dong and Fu found that European-Americans and Chinese contributors can tag images diferently [8]. 
    8. War versus inspirational in forrest gump: Cultural effects in tagging communities \cite{DBLP:conf/icwsm/DongSSTR12}

subjective judgments can be afected by con- tributor attitudes [26]


Nguyen et al. [23] showed that gender detection is difficult because of implicit associations and social constructions that take place in the annotation process.
    23. Why gender and age prediction from tweets is hard: Lessons from a crowdsourcing experiment \cite{DBLP:conf/coling/NguyenTDGTMJ14}


These issues are especially relevant when crowdsourcing is used to label data that are used by machine learning models


While the issue of dataset bias has been extensively investigated from the perspective of the data samples themselves (e.g., [2, 19, 27, 39, 42])
    2. Women also Snowboard: Overcoming Bias in Captioning Models \cite{DBLP:conf/eccv/HendricksBSDR18}
    19. Undoing the damage of dataset bias \cite{DBLP:conf/eccv/KhoslaZMET12}
    27. A survey on transfer learning \cite{DBLP:journals/tkde/PanY10}
    39. A deeper look at dataset bias \cite{DBLP:series/acvpr/TommasiPCT17}
    42. Men also like shopping: Reducing gender bias amplification using corpus-level constraints \cite{DBLP:conf/emnlp/ZhaoWYOC17} 


prior works so far have only hinted and encouraged researchers to study the impact of biases in contributor demographics in crowdsourcing (e.g., [34, 38]).
    34. Turkers, scholars, arafat and peace: Cultural communities and algorithmic gold standard \cite{DBLP:conf/cscw/SenGGHLNRWH15}
    38. Simulation Experiments On (The Absence of) Ratings Bias in Reputation Systems \cite{DBLP:journals/pacmhci/Thebault-Spieker17}




Our framework considers these human factors to enable requesters to obtain unbiased contributor samples.


Our study shows that accuracy and acceptance rates alone are not appropriate indicators of training data quality and that the human behind the label must also be considered in order to mitigate issues of bias that can limit the performance of machine learning models used in the wild.


Among many possible improvements to our framework, one of them is adding the ability for it to automatically identify demographics that need to be optimized.


In any multi-objective optimization problem, conflicting states are likely to occur. This motivated our choice of applying Pareto-optimal selection so that these trade-offs could be accounted for. 


As observed in our experiment, there are trade-offs between labeling with less bias and completing the task faster.


---
In hand with the challenges for running controlled experiments and studies on crowdsourcing platforms are the potential biases that could emerge from the lack of complete control of [xxx] that could potentially harm the outcomes.
%
This could range from, for example, [some "straighforward" things that can be controlled] to more [sophisitcated ones].
---
%%% -------------------------------------- %%% %%% -------------------------------------- %%% 





---

Over the years, a vast body of work assessed the feasibility of growing the scope of crowdsourcing \cite{Paolacci2010RunningEO,Buhrmester2011AmazonsMT,DBLP:journals/sigkdd/MasonW09,Schnoebelen2010UsingAM,DBLP:conf/icse/SunS16,Crump2013}, expanding its application beyond serving as a tool to create machine learning datasets 
[citations]. 
%
Paid crowd work, through crowdsourcing platforms, establishes as a mechanism for running user studies \cite{DBLP:conf/chi/KitturCS08,Buhrmester2011AmazonsMT,DBLP:conf/icse/SunS16}, experiments \cite{Crump2013,Paolacci2010RunningEO,DBLP:journals/sigkdd/MasonW09,Schnoebelen2010UsingAM,DBLP:conf/hcomp/WuQ17,DBLP:conf/cscw/KitturNBGSZLH13,DBLP:conf/ht/GadirajuYB17,DBLP:conf/naacl/LiuSBLLW16,DBLP:conf/chi/SampathRI14,Wilson2016WWW,ramirez2019,maddalena2016crowdsourcing,krishna2016embracing} and even complex work that initially does not fit in the microtask market \cite{DBLP:conf/uist/KitturSKK11,DBLP:conf/uist/AhmadBMK11,DBLP:conf/cscw/KulkarniCH12}.
%
Naturally, the set of challenges also increases along with the scope and ambition of crowdsourcing projects.
%
The potential size of the design space, along with the individual and environmental biases \cite{DBLP:conf/chi/BarbosaC19,DBLP:conf/lrec/BalahurSKZGHPB10,DBLP:conf/ht/ChengC13,eickhoff2018cognitive,DBLP:conf/coling/NguyenTDGTMJ14,DBLP:conf/cscw/SenGGHLNRWH15}, and the limitations of crowdsourcing platforms \cite{Qarout2019PlatformRelatedFI,DBLP:conf/www/Paritosh12}, makes it difficult to run controlled crowdsourcing experiments (e.g., systematically evaluating task design alternatives).





This goes against one of the benefits of crowdsourcing when compared to laboratory settings; it releases researchers from trading off sample size and gives access to a large and diverse pool of workers instead \cite{DBLP:conf/chi/KitturCS08}.

---


==> sections/tmp-related.tex <==
% crowdsourcing tooling available.

% 1. domain-specific tooling: CrowdRev, Soilent, crowd databases, etc.
% 2. general purpose
    % tools for interdepedent tasks: crowdforge, turkomatic, etc, etc
    % programming







%%% -------------------------------------- %%% %%% -------------------------------------- %%% 

% 1. domain specific tooling
Soylent \cite{DBLP:conf/uist/BernsteinLMHAKCP10} is a word processor that embeds crowdsourcing to shorten, proofread or edit a document, and introduced a programming design pattern called find-fix-verify that splits the complex work into stages.


We thus present Soylent, a word processing interface that enables writers to call on Mechanical Turk workers to shorten, proofread, and otherwise edit parts of their documents on demand

To improve worker quality, we introduce the Find-Fix-Verify crowd programming pattern, which splits tasks into a series of generation and re- view stages



Soylent is comprised of three main components: 
    Shortn, a text shortening service
 
    Crowdproof, a human-powered spelling and grammar checker that finds problems Word misses,
 
    The Human Macro, an interface for offloading arbi- trary word processing tasks such as formatting cita- tions or finding appropriate figures.


The main contribution of this paper is the idea of embed- ding paid crowd workers in an interactive user interface to support complex cognition and manipulation tasks on demand.

Soylent is a prototype crowdsourced word processing inter- face with three features: shortening, proofreading, and arbi- trary macro tasks via human-language input.

we propose the Find-Fix-Verify pattern as one method of programming crowds to reliably complete open-ended tasks that directly edit the user’s data

The Find-Fix-Verify pattern separates open-ended tasks into three stages where each worker can make a clear con- tribution.


Crowdrev \cite{CrowdRev2018}


SciCrowd \cite{DBLP:conf/criwg/CorreiaSPF18}

The system combines automatic data indexing and crowd-based processing of data for detecting topic evolution by fostering a knowledge base of concepts, methods, and results categorized according to the particular needs of each field.

SciCrowd is a system prototype based on a crowd-enabled model [4] that supports the entire process of research data analysis

Our approach to extract information from public data sources is based on a previous proposal for a hybrid human-computer scientific information extraction pipeline



%%%
CrowdDB \cite{DBLP:conf/sigmod/FranklinKKRX11}

CrowdDB models crowdsourcing as an extension to relational databases, providing annotations to traditional SQL queries that trigger the SQL runtime to crowdsource database cleansing tasks [14]. The SQL runtime is crowdsourcing- aware, so that the SQL’s query planner can minimize opera- tions that would otherwise be very expensive. Unlike AUTO- MAN, CrowdDB is not a general platform for computing, and relies on majority voting as its sole quality control mechanism.


CrowdDB uses human input via crowdsourcing to process queries that neither database systems nor search engines can adequately answer. It uses SQL both as a language for posing complex queries and as a way to model data

Crowdsourcing databases extend the capabilities of database systems to allow answering queries via crowd workers to aid data cleansing pipelines. 

for CrowdDB, we develop crowd-based implementations of query operators for finding and comparing data, while relying on the traditional relational query operators to do the heavy lifting for bulk data manipulation and processing.

Our approach leverages schema information to support the automatic generation of effective user interfaces for crowdsourced tasks.

CrowdSQL extends SQL’s data definition language to enable application developers to annotate tables with information that helps in user interface creation.




%%%

Deco \cite{DBLP:conf/cikm/ParameswaranPGPW12}

Deco is a comprehensive system for answering declarative queries posed over stored relational data together with data obtained on- demand from the crowd


Several recent data-oriented systems have used a declarative ap- proach to leverage crowdsourced data [1, 7, 10, 16, 17]. Among those systems
    1: Answering search queries with crowdsearcher
    2: Declarative platform for data sourcing games
    10: CrowdDB: Answering queries with crowdsourcing
    16: Human-powered sorts and joins \cite{DBLP:journals/pvldb/MarcusWKMM11}
    17: CyLog/Crowd4U: A declarative platform for complex data-centric crowdsourcing


%%%
CrowdQ: Crowdsourced Query Understanding \cite{DBLP:conf/cidr/DemartiniTKF13}

%%%
Human-powered sorts and joins \cite{DBLP:journals/pvldb/MarcusWKMM11}

%%%
CyLog/Crowd4U: A declarative platform for complex data-centric crowdsourcing \cite{DBLP:journals/pvldb/MorishimaSMAF12}

%%% -------------------------------------- %%% %%% -------------------------------------- %%% 




%%% -------------------------------------- %%% %%% -------------------------------------- %%% 
% 2.1 tools for interdepedent tasks: crowdforge, turkomatic, etc, etc
% these tools have in common that they focus on complex interdepedent tasks and they propose a fixed workflow.

---
Several approaches have been proposed to manage complex problems that partition into interdependent tasks. Inspired by the MapReduce programming paradigm \cite{DBLP:conf/osdi/DeanG04}, CrowdForge \cite{DBLP:conf/uist/KitturSKK11} offers a framework to allow solving complex problems via a combination of partition, map and reduce tasks.
%
Jabberwocky \cite{DBLP:conf/uist/AhmadBMK11} is a social computing stack that offers three core components to tackle complex (and potentially interdependent) tasks. Dormouse represents the foundations of Jabberwocky, and it acts as the runtime that can process human (and hybrid) computation, offering for cross-platform capabilities (e.g., going beyond Amazon Mechanical Turk). The ManReduce layer is similar to CrowdForge but implemented as a framework for the Ruby programming language, allowing map and reduce steps to be executed by either crowd or machines. Finally, Jabberwocky offers a high-level procedural language called Dog that compiles down to ManReduce programs. 
---

[from CrowdLang:]
Several programming frameworks inspired by the MapReduce [14] program- ming metaphor have been proposed to coordinate arbitrary dependencies between interdependent tasks. These frameworks model complex problems as a sequence of partitioning, mapping, and reducing subtasks

%%
CrowdForge \cite{DBLP:conf/uist/KitturSKK11} propose a general framework inspired by MapReduce, solving a complex problem by a combination of partition, map, and reduce tasks. 


%%
Jabberwocky \cite{DBLP:conf/uist/AhmadBMK11} extended this idea (CrowdForge) by providing an additional human and resource management system for integrating workforces from different markets, as well as a high-level procedural programming language

% Jabberwocky provides a human-computation stack on top of a MapReduce-like parallel programming framework called ManReduce [1]. A Ruby DSL called Dog eases programmer interaction with a resource-management layer called Dormouse, which does the actual scheduling of tasks on ManReduce. Jabberwocky uses a fixed, optional quality con- trol scheme based on majority voting and a fixed pricing scheme.

a social computing stack that consists of three components: a human and machine resource management system called Dormouse, a parallel program- ming framework for human and machine computation called ManReduce, and a high-level programming language on top of ManReduce called Dog.

Dormouse is designed to enable cross-platform programming languages for social computation, so, for example, programs written for Mechanical Turk can also run on other crowdsourcing platforms.


We show that the unique properties of Dormouse enable elegant programming models for com- plex and useful problems, and we propose two such frameworks: ManReduce and Dog

ManReduce is a framework for combining human and machine computation into an intuitive parallel data flow

Dog is a high-level procedural language written on top of ManReduce that focuses on expressivity and reuse

The ManReduce framework is written in Ruby. [though they said they are working on Python and Java]





%%%
Turkomatic \cite{DBLP:conf/cscw/KulkarniCH12} is a system that propose a general-purpose meta-algorithm consisting of price, divide, solve and merge steps where the crowd helps in producing the algorithm that will run in AMT.

% Turkomatic aims to crowdsource an entire computation, including the “programming” of the task [19]. Tasks are provided to the system in plain English, and the Turkomatic runtime proceeds in two steps: a map step and a reduce step. In the map step, workers provide an execution plan, which is then carried out in the reduce step. Like AUTOMAN, Turko- matic can be used to construct arbitrarily complex compu- tations. However, Turkomatic does not handle budgeting or quality control, and also cannot be integrated with a conventional programming language.


Can the crowd help design such workflows? This paper presents Turkomatic, a tool that recruits crowd workers to aid requesters in planning and solving complex jobs

Turkomatic uses a novel meta-workflow to induce the crowd to design and execute workflows.

The system executes a continuous price-divide-solve loop that asks workers to recursively divide complex steps into simpler ones until they are at an appropriately simple level, then to solve them


While workers decompose and solve tasks, requesters can view the status of worker-designed workflows in real time; intervene to change tasks and solutions; and request new solutions to subtasks from the crowd

Turkomatic is based on a price-divide-solve algorithm that guides workers through the steps of decomposing and solving tasks; and on generic task templates that are instantiated with particular task contexts



----
Turkomatic \cite{DBLP:conf/cscw/KulkarniCH12} also focuses on supporting requesters in crowdsourcing complex tasks, but unlike previous approaches, it allows the crowd to play an active role in decomposing the problem into the set of interdependent components. Turkomatic operates using a divide-and-conquer loop where workers actively refine the input problem (supervised by requesters) into subtasks that run on AMT, where a set of generic task templates are instantiated accordingly.
----






%%%
Platemate \cite{DBLP:conf/uist/NoronhaHZG11} suggest a “divide-and-conquer” management framework inspired by corporate hierarchies.


%%%
Zhang et al. \cite{DBLP:conf/chi/ZhangLMGPH12}, for example, propose a system that exploits a self-organizing crowd to solve a planning under constraints problem.



%%%
Knowledge accelerator workflow \cite{DBLP:conf/chi/HahnCKK16}.





%%% -------------------------------------- %%% %%% -------------------------------------- %%% 








%%% -------------------------------------- %%% %%% -------------------------------------- %%% 
% 2.2 programming
%%
Turkit, toolkit and presents an iterative improvements algorithm where workers build and improve on previous answers \cite{DBLP:conf/uist/LittleCGM10}. 

imperative programming framework TurKit

TurKit is a toolkit for exploring human computation algo- rithms on Mechanical Turk


---
Turkit \cite{DBLP:conf/uist/LittleCGM10} is a JavaScript programming toolkit for implementing human computation algorithms that run on Amazon Mechanical Turk, offering functions that interface with AMT and introducing the crash-and-rerun programming model for building robust crowdsourcing scripts.
---



CrowdLang: A Programming Language for the Systematic Exploration of Human Computation Systems \cite{DBLP:conf/socinfo/MinderB12}.

a general-purpose framework and programming language for interweaving human and machine computation.

In this paper we present the CrowdLang programming framework for engineering complex com- putation systems incorporating large crowds of networked humans and machines with a library of known interaction patterns.

The evaluation shows that CrowdLang is able to simply explore a large design space of possible problem-solving programs with the simple varia- tion of the used abstractions


Human computation systems are often the result of extensive lengthy trial-and-error refinements. What we lack is an approach to systematically engineer solutions based on past successful patterns.


Relying on [4] this paper considers human computation as computation that is carried out by humans and human computation systems as "paradigms for utilizing human processing power to solve problems that computers cannot yet solve"
    4. Law, E., Ahn, L.: Human computation. Synthesis Lectures on Artificial Intelligence and Machine Learning 5(3) (2011) 1–121


CrowdLang supports cross-platform workforce integration, the management of human computer latency, and incorporates abstractions for group decisions, contests, and collaborative interaction patterns



The framework consists of three major components: (1) The CrowdLang Library simplifies the design of new human computation systems. It supports the seamless reuse of existing interaction patterns by providing an extensible pro- gramming library.

(2) The CrowdLang Engine addresses the technical challenges of executing hu- man computation algorithms by managing the crowd latency (waiting for human response), debugging human computation code, and the re-executing of human computation after exceptions.

(3) The CrowdLang Integrator integrates different execution platforms such as micro-task markets and games with a purpose

---
CrowdLang \cite{DBLP:conf/socinfo/MinderB12} is a framework and programming language for human and machine computation, relying on three core components to allow requesters to implement complex crowdsourcing workflows. The first element is a programming library that encapsulates operators and reusable human computation workflows (e.g., find-fix-verify \cite{DBLP:conf/uist/BernsteinLMHAKCP10}, iterative improvements \cite{DBLP:conf/uist/LittleCGM10}), then the engine is responsible for orchestrating and running the human computation algorithms. Finally, the integration layer bridges CrowdLang with distinct crowdsourcing platforms for cross-platform support. 
---





%%
AUTOMAN: A Platform for Integrating Human-Based and Digital Computation \cite{DBLP:conf/oopsla/BarowyCBM12}

The lack of complete automation makes it difficult to orchestrate complex or interrelated tasks

The first fully automatic crowdprogramming system. AUTOMAN integrates human- based computations into a standard programming language as ordinary function calls, which can be intermixed freely with traditional functions


An AUTOMAN program specifies a confidence level for the overall computation and a budget. The AUTOMAN runtime system then transparently manages all details necessary for schedul- ing, pricing, and quality control.

AUTOMAN is a domain-specific language embedded in Scala

AUTOMAN’s goal is to abstract away the details of crowdsourcing so that human computation can be as easy to invoke as a conventional function.

----
Similar to Turkit, AUTOMAN \cite{DBLP:conf/oopsla/BarowyCBM12} embeds crowdsourcing capabilities into a programming language (Scala in this case). However, it also offers features to automatically manage pricing, quality control, and scheduling of crowdsourcing tasks.
----


%%%
Reactive crowdsourcing \cite{DBLP:conf/www/BozzonBCM13}
Bozzon et al.  propose a framework and a reactive execution environment for modelling and controlling human computation algorithms.





%%%
TurkServer: Enabling Synchronous and Longitudinal Online Experiments \cite{DBLP:conf/hcomp/MaoCGPPZ12}.


---
Closest to our work is the TurkServer platform \cite{DBLP:conf/hcomp/MaoCGPPZ12} that enables researchers to run behavioral studies and experiments on Amazon Mechanical Turk.

Closest to our work is the TurkServer platform \cite{DBLP:conf/hcomp/MaoCGPPZ12} that enables researchers to run behavioral studies and experiments on Amazon Mechanical Turk.


As can be noticed, these works illustrate that substantial efforts have been devoted to offering solutions that sit on top of crowdsourcing platforms. However, for systematically evaluating multiple task designs, the above tools still demands substantial effort from requesters (e.g., programming the complete workflows or experiments).
%
In this context, we find the TurkServer platform \cite{DBLP:conf/hcomp/MaoCGPPZ12} to be closely related to our work. TurkServer offers builtin features that enable researchers to run controlled experiments on Amazon Mechanical Turk.  However, requesters need to program their experiments since TurkServer is a JavaScript web-based framework.
%
Even though programming frameworks give full flexibility to researchers, CrowdHub aims to offer a paradigm that blends flexibility with productivity. With CrowdHub, we propose an easy-to-use platform that allows researchers to focus on designing the experiments via a diagramming interface, reducing the programming efforts that current tooling would require.

---








%%


%%% -------------------------------------- %%% %%% -------------------------------------- %%% 






 












